Missing data imputation for noisy time-series data and applications in healthcare

Healthcare time series data is vital for monitoring patient activity but often contains noise and missing values due to various reasons such as sensor errors or data interruptions. Imputation, i.e., filling in the missing values, is a common way to deal with this issue. In this study, we compare imputation methods, including Multiple Imputation with Random Forest (MICE-RF) and advanced deep learning approaches (SAITS, BRITS, Transformer) for noisy, missing time series data in terms of MAE, F1-score, AUC, and MCC, across missing data rates (10 % - 80 %). Our results show that MICE-RF can effectively impute missing data compared to deep learning methods and the improvement in classification of data imputed indicates that imputation can have denoising effects. Therefore, using an imputation algorithm on time series with missing data can, at the same time, offer denoising effects.

==> note.tex <==
- univariate: TIMEMIXER (2024), ITRANSFORMER(2024), MODERNTCN (2024), ETSformer (2023), brits(2018), Random Forest,
+ 2 - 3 datasets: consider: noisy, non-noisy
- multivariate: TIMEMIXER, ITRANSFORMER, MODERNTCN, ETSformer (2023), brits

uncertainty quantification, explainability


datasets: 
https://datasets.simula.no/
univariate:
psykose (patient 1, control1)
depresjon-dataset (control, patient)


saits (2023), transformer, TimesNet, CSDI, US-GAN, GP-VAE, BRITS, M-RNN, LOCF

https://docs.pypots.com/en/latest/pypots.imputation.html

https://docs.pypots.com/en/latest/?_gl=1*iehw19*_ga*MTk1MTYxNTAzLjE3MjY0OTYyMDc.*_ga_TLYTE74XVR*MTcyNjQ5NjIwNy4xLjEuMTcyNjQ5Njc0OC4wLjAuMA..

https://github.com/WenjieDu/BrewPOTS/blob/main/PyPOTS_Imputation.ipynb


imputation algorithms that can only run on multivariate data: CSDI (2021 Conditional Score-based Diffusion Models for Probabilistic Time Series Imputation)
@article{vu2023conditional,
  title={Conditional expectation with regularization for missing data imputation},
  author={Vu, Mai Anh and Nguyen, Thu and Do, Tu T and Phan, Nhan and Chawla, Nitesh V and Halvorsen, P{\aa}l and Riegler, Michael A and Nguyen, Binh T},
  journal={arXiv preprint arXiv:2302.00911},
  year={2023}
}

@article{nguyen2022dper,
  title={DPER: direct parameter estimation for randomly missing data},
  author={Nguyen, Thu and Nguyen-Duy, Khoi Minh and Nguyen, Duy Ho Minh and Nguyen, Binh T and Wade, Bruce Alan},
  journal={Knowledge-Based Systems},
  volume={240},
  pages={108082},
  year={2022},
  publisher={Elsevier}
}
@inproceedings{riegler2023scopesense,
  title={ScopeSense: An 8.5-month sport, nutrition, and lifestyle lifelogging dataset},
  author={Riegler, Michael A and Thambawita, Vajira and Chatterjee, Ayan and Nguyen, Thu and Hicks, Steven A and Telle-Hansen, Vibeke and Pettersen, Svein Arne and Johansen, Dag and Jain, Ramesh and Halvorsen, P{\aa}l},
  booktitle={International Conference on Multimedia Modeling},
  pages={502--514},
  year={2023},
  organization={Springer International Publishing Cham}
}

==> note_table.tex <==
%Table MAE comparison 
\begin{table}[h!]
\setlength{\tabcolsep}{3pt} % Adjust column spacing (default is 6pt)
\renewcommand{\arraystretch}{1.25} % Adjust row height (1.0 is the default)
\centering
\caption{Result of experiment - dataset Psykose with epoch=10, n\_layers=1}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Missing rate} & \textbf{MICE + RF} & \textbf{BRITS} & \textbf{Transformer} & \textbf{SAITS} \\ \hline
10.0  & 0.352  & 0.648  & 0.699  & 0.533  \\ \hline
20.0  & 0.367  & 0.670  & 0.642  & 0.544  \\ \hline
30.0  & 0.382  & 0.645  & 0.677  & 0.549  \\ \hline
40.0  & 0.399  & 0.663  & 0.727  & 0.557  \\ \hline
50.0  & 0.417  & 0.682  & 0.665  & 0.559  \\ \hline
60.0  & 0.438  & 0.696  & 0.744  & 0.576  \\ \hline
70.0  & 0.478  & 0.683  & 0.737  & 0.577  \\ \hline
80.0  & 0.540  & 0.694  & 0.779  & 0.597  \\ \hline
\end{tabular}
\label{table:mae_psykose-1nlayer}

\end{table}

\begin{table}[h!]
\centering
\setlength{\tabcolsep}{3pt} % Adjust column spacing (default is 6pt)
\renewcommand{\arraystretch}{1.25} % Adjust row height (1.0 is the default)
\caption{Result of experiment - dataset Psykose with epoch=10, n\_layers=2}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Missing rate} & \textbf{MICE + RF} & \textbf{BRITS} & \textbf{Transformer} & \textbf{SAITS} \\ \hline
10.0  & 0.352  & 0.655  & 0.959  & 0.583  \\ \hline
20.0  & 0.366  & 0.657  & 1.036  & 0.591  \\ \hline
30.0  & 0.381  & 0.659  & 0.903  & 0.592  \\ \hline
40.0  & 0.396  & 0.672  & 0.926  & 0.596  \\ \hline
50.0  & 0.418  & 0.678  & 0.944  & 0.595  \\ \hline
60.0  & 0.442  & 0.680  & 1.017  & 0.591  \\ \hline
70.0  & 0.478  & 0.678  & 0.977  & 0.616  \\ \hline
80.0  & 0.538  & 0.696  & 0.980  & 0.634  \\ \hline
\end{tabular}
\label{table:mae_psykose-2nlayer}

\end{table}

\begin{table}[h!]
\setlength{\tabcolsep}{3pt} % Adjust column spacing (default is 6pt)
\renewcommand{\arraystretch}{1.25} % Adjust row height (1.0 is the default)
\centering
\caption{Result of experiment - dataset Depresjon with epoch=10, n\_layers=1}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Missing rate} & \textbf{MICE + RF} & \textbf{BRITS} & \textbf{Transformer} & \textbf{SAITS} \\ \hline
10.0  & 0.290  & 0.592  & 0.646  & 0.467  \\ \hline
20.0  & 0.300  & 0.587  & 0.657  & 0.478  \\ \hline
30.0  & 0.311  & 0.574  & 0.677  & 0.479  \\ \hline
40.0  & 0.326  & 0.625  & 0.614  & 0.485  \\ \hline
50.0  & 0.341  & 0.602  & 0.614  & 0.487  \\ \hline
60.0  & 0.363  & 0.629  & 0.699  & 0.490  \\ \hline
70.0  & 0.397  & 0.621  & 0.707  & 0.492  \\ \hline
80.0  & 0.445  & 0.616  & 0.656  & 0.500  \\ \hline
\end{tabular}
\label{table:mae_depresjon-1nlayer}

\end{table}

\begin{table}[h!]
\centering
\setlength{\tabcolsep}{3pt} % Adjust column spacing (default is 6pt)
\renewcommand{\arraystretch}{1.25} % Adjust row height (1.0 is the default)
\caption{Result of experiment - dataset Depresjon with epoch=10, n\_layers=2}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Missing rate} & \textbf{MICE + RF} & \textbf{BRITS} & \textbf{Transformer} & \textbf{SAITS} \\ \hline
10.0 & 0.286 & 0.587 & 0.866 & 0.499 \\ \hline
20.0 & 0.301 & 0.583 & 0.811 & 0.509 \\ \hline
30.0 & 0.313 & 0.605 & 0.762 & 0.507 \\ \hline
40.0 & 0.324 & 0.623 & 0.833 & 0.522 \\ \hline
50.0 & 0.342 & 0.603 & 0.792 & 0.514 \\ \hline
60.0 & 0.363 & 0.629 & 0.838 & 0.527 \\ \hline
70.0 & 0.395 & 0.624 & 0.821 & 0.538 \\ \hline
80.0 & 0.446 & 0.610 & 0.824 & 0.545 \\ \hline
\end{tabular}
\label{table:mae_depresjon-2nlayer}
\end{table}
